AKiRa: Augmentation Kit on Rays for optical video generation

Recent advances in text-conditioned video diffusion have greatly improved video quality. However, these methods offer limited or sometimes no control to users on camera aspects, including dynamic camera motion, zoom, distorted lens and focus shifts. These motion and optical aspects are crucial for adding controllability and cinematic elements to generation frameworks, ultimately resulting in visual content that draws focus, enhances mood, and guides emotions according to filmmakers' controls. In this paper, we aim to close the gap between controllable video generation and camera optics. To achieve this, we propose AKiRa (Augmentation Kit on Rays), a novel augmentation framework that builds and trains a camera adapter with a complex camera model over an existing video generation backbone. It enables fine-tuned control over camera motion as well as complex optical parameters (focal length, distortion, aperture) to achieve cinematic effects such as zoom, fisheye effect, and bokeh. Extensive experiments demonstrate AKiRa's effectiveness in combining and composing camera optics while outperforming all state-of-the-art methods. This work sets a new landmark in controlled and optically enhanced video generation, paving the way for future optical video generation methods.

==> tab/optical.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{\begin{tabular}{@{}l ccc@{\hspace{3pt}}c@{\hspace{3pt}}c@{}}
\toprule
\multirow{2}{*}{\textbf{Method}}                & \multirow{2}{*}{\textbf{ZoomSim} $\uparrow$} & \multirow{2}{*}{\textbf{DistortSim} $\uparrow$} & \multicolumn{3}{c}{\textbf{FocusArea}} \\ 
      &  &   & $\alpha$=$0$ & $\alpha$=$30$ & $\alpha$=$100$ \\
\midrule
AnimateDiff~\cite{guo2023animatediff} &                     $0.00$ &                      $0.00$ & $0.90$ & - & -\\
CameraCtrl~\cite{he2024cameractrl}   &                     $78.98$ &                     $62.13$ & $0.69$ & - & -\\
AKiRa (ours)                         & \cellcolor{tabfirst}$86.82$ & \cellcolor{tabfirst}$81.19$ & $0.72$ & $0.64$ & $0.61$ \\
\bottomrule 
\end{tabular}}
\caption{\textbf{Optical comparison.} Comparison of AKiRa and CameraCtrl~\cite{he2024cameractrl} with Animatediff~\cite{guo2023animatediff} backbone on WebVid
dataset, evaluating optical coherence (zoom, distortion and bokeh). \colorbox{tabfirst}{Best}.}
\label{tab:optical}
\end{table}



==> tab/user+ablation.tex <==
\begin{figure*}[htbp]
% \centering
%   \begin{minipage}[b]{\textwidth}
%   %\begin{figure*}[t]
%     \centering
%     \includegraphics[width=\linewidth]{fig/dolly.pdf}
%     \captionof{figure}{\textbf{Comparison of dolly zoom.} Comparison of the dolly zoom effect using SVD (I2V)~\cite{blattmann2023svd} backbone between \akira, the reference clip from \emph{JAWS} (\emph{Spielberg, 1975}), and CameraCtrl\cite{he2024cameractrl}.
%     \todo{Change to vertigo examples}}
%     \label{fig:dolly}
% %\end{figure*}
% \end{minipage}
% \\
\centering
  \begin{minipage}[b]{0.62\textwidth}
    \centering
    \resizebox{\textwidth}{!}{
    \input{tab/user_study}  
    }
    \captionof{table}{\textbf{Results of user study.} Proportion of participants ranking each method as 1st for each criterion: the quality of the video (\emph{Video}), text-to-video consistency (\emph{Text-to-video}), motion fidelity, and optical coherence (\emph{Zoom}, \emph{Distortion}, \emph{Bokeh}). \colorbox{tabfirst}{First best} and \colorbox{tabsecond}{second best}.}
    \label{tab:user-study}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.34\textwidth}
    \centering
    \resizebox{\textwidth}{!}{
    \input{tab/ablation}  
  }
 
    \captionof{table}{\textbf{Ablation of augmentations.} \akira trained on Animatediff~\cite{guo2023animatediff} with all combinations of the proposed data augmentation kit.}
    \label{tab:ablation}
  \end{minipage}
  
\end{figure*}

==> tab/vic_user_ablation_extra.tex <==
%{{\renewcommand{\arraystretch}{1.2} 

\begin{figure*}[htbp]
% \centering
%   \begin{minipage}[b]{\textwidth}
%   %\begin{figure*}[t]
%     \centering
%     \includegraphics[width=\linewidth]{fig/dolly.pdf}
%     \captionof{figure}{\textbf{Comparison of dolly zoom.} Comparison of the dolly zoom effect using SVD (I2V)~\cite{blattmann2023svd} backbone between \akira, the reference clip from \emph{JAWS} (\emph{Spielberg, 1975}), and CameraCtrl\cite{he2024cameractrl}.
%     \todo{Change to vertigo examples}}
%     \label{fig:dolly}
% %\end{figure*}
% \end{minipage}
% \\
\centering
  \begin{minipage}[b]{0.65\textwidth}
    \centering
    \footnotesize{
    %\resizebox{\textwidth}{!}{
    \input{tab/user_study}  
    }
    \captionof{table}{\textbf{Results of user study.} \% participants ranking each method as 1st for:  \emph{Video} quality, \emph{Text-to-video} consistency, motion fidelity, and optical coherence (\emph{Zoom}, \emph{Distortion}, \emph{Bokeh}). %\colorbox{tabfirst}{First best} and \colorbox{tabsecond}{second best}.
    }
    \label{tab:user-study} 
    %\\
    \footnotesize{
        %\resizebox{\textwidth}{!}
        {\begin{tabular}{@{}l ccc@{\hspace{3pt}}c@{\hspace{3pt}}c@{}}
        \toprule
        \multirow{2}{*}{\textbf{Method}}                & \multirow{2}{*}{\textbf{ZoomSim} $\uparrow$} & \multirow{2}{*}{\textbf{DistortSim} $\uparrow$} & \multicolumn{3}{c}{\textbf{FocusArea}} \\ 
              &  &   & $\alpha$=$0$ & $\alpha$=$30$ & $\alpha$=$100$ \\
        \midrule
        AnimateDiff~\cite{guo2023animatediff} &                     $0.00$ &                      $0.00$ & $0.90$ & - & -\\
        CameraCtrl~\cite{he2024cameractrl}   &                     $78.98$ &                     $62.13$ & $0.69$ & - & -\\
        AKiRa (ours)                         & \cellcolor{tabfirst}$86.82$ & \cellcolor{tabfirst}$81.19$ & $0.72$ & $0.64$ & $0.61$ \\
        \bottomrule 
        \end{tabular}}}
        \captionof{table}{\textbf{Optical comparison.} Comparison of AKiRa and CameraCtrl~\cite{he2024cameractrl} with Animatediff~\cite{guo2023animatediff} backbone on WebVid
        dataset, evaluating optical coherence (zoom, distortion and bokeh). \colorbox{tabfirst}{First best} and \colorbox{tabsecond}{second best}.}
        \label{tab:optical}
%
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.28\textwidth}
    \centering
    \resizebox{\textwidth}{!}{
    \input{tab/ablation}  
  }
 
    \captionof{table}{\textbf{Ablation of augmentations.} \akira trained on Animatediff~\cite{guo2023animatediff} with all combinations of the proposed data augmentation kit.}
    \label{tab:ablation}
  \end{minipage}
  
\end{figure*}
